CadVLM: Bridging Language and Vision in the Generation of Parametric CAD Sketches

Parametric Computer-Aided Design (CAD) is central to contemporary mechanical design. However, it encounters challenges in achieving precise parametric sketch modeling and lacks practical evaluation metrics suitable for mechanical design. We harness the capabilities of pre-trained foundation models, renowned for their successes in natural language processing and computer vision, to develop generative models specifically for CAD. These models are adept at understanding complex geometries and design reasoning, a crucial advancement in CAD technology. In this paper, we propose CadVLM, an end-to-end vision language model for CAD generation. Our approach involves adapting pre-trained foundation models to manipulate engineering sketches effectively, integrating both sketch primitive sequences and sketch images. Extensive experiments demonstrate superior performance on multiple CAD sketch generation tasks such as CAD autocompletion, CAD autoconstraint, and image conditional generation. To our knowledge, this is the first instance of a multimodal Large Language Model (LLM) being successfully applied to parametric CAD generation, representing a pioneering step in the field of computer-aided mechanical design.

==> sections/abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
% Parametric Computer-Aided Design (CAD) is the dominant paradigm for modern mechanical design. Training generative models to reason and generate parametric CAD can dramatically speed up design workflows. Pretrained foundation models have shown great success in natural language processing and computer vision. The cross-domain knowledge embedded in these models holds significant potential for understanding geometry and performing complex reasoning about design. In this work, we develop generative models for CAD by leveraging pre-trained language models and apply them to manipulate engineering sketches.
% Our results demonstrate that models pre-trained on natural language can be fine-tuned on engineering sketches and achieve remarkable performance in various CAD generation scenarios.
Parametric Computer-Aided Design (CAD) is central to contemporary mechanical design. We harness the capabilities of pre-trained foundation models, renowned for their successes in natural language processing and computer vision, to develop generative models specifically for CAD. These models are adept at understanding complex geometries and design reasoning, a crucial advancement in CAD technology. In this paper, we propose CadVLM, an end-to-end vision language model for CAD generation. Our approach involves adapting pre-trained foundation models to manipulate engineering sketches effectively, integrating both sketch primitive sequences and sketch images. Extensive experiments demonstrate superior performance on multiple CAD sketch generation tasks such as CAD autocompletion, CAD autoconstraint, and image conditional generation. To our knowledge, this is the first instance of a multimodal Large Language Model (LLM) being successfully applied to parametric CAD generation, representing a pioneering step in the field of computer-aided mechanical design. The code is available at \href{https://anonymous.4open.science/r/CadVLM}{https://anonymous.4open.science/r/CadVLM}.
\end{abstract}

==> sections/background.tex <==
\section{Background}
\label{sec:background}
\begin{figure*}[ht]
    \centering
    \includegraphics[scale=0.54]{cvpr2023-author_kit-v1_1-1/latex/sections/architecture.pdf}
    \caption{\textbf{CadVLM model architecture and training objectives} for CAD autoconstraint. We propose a unified vision-language model capable of outputting both autocompleted sketch images and sketch primitives. The inputs are paired incomplete sketch primitives and images, which are encoded by pre-trained text encoder and image encoder correspondingly. Aligned by image-text contrastive(ITC) loss, the concatenation of image embedding and text embedding then will be input to text-grounded image decoder and image-grounded text decoder. The image decoder is trained with image decoding loss between autocompleted sketch images and ground-truth sketch images. The text decoder is trained with a language modeling(LM) loss to generate autocompleted primitive.}
    \label{fig:architecture}
    \vspace{-4mm}
\end{figure*}
% \textbf{Engineering Sketch Definition.} Sketches, varying from millimeters to meters, are centered at the origin within a 1-meter width bounding box to reduce ambiguity. Each sketch is comprised of both a sequence of primitives, $\mathcal{S}$, and a sequence of constraints, $\mathcal{C}$. 
% Continuous primitive parameters are converted to discrete variables through 6-bit uniform quantization for flexible modeling of diverse shapes. Normalization and quantization for primitive parameters are similar to ~\cite{seff2021vitruvion}. 
% % We aim to investigate the procedure for steering a pre-trained foundational language model on parametric CAD sketches. Each sketch is comprised of a sequence of entities: 
% Each sketch primitive is formatted as $\mathcal{S} = (e_1, e_2, ..., e_m),$ 
% where $m$ is the number of entities in the sketch. Each entity $e_i$ is represented by position parameters $(p_1,..., p_k)$, where $p_k$ represents the normalized coordinate parameters of the points forming the entity. We have three types of entities: line, arc, and circle. We represent them with two, three, and four points respectively as in~\cite{willis2021engineering} allowing each sketch to be viewed as a sequence of tokens. 
% Constraint is represented similarly as primitive, which is formatted as $\mathcal{C} = (c_1, c_2, ...).$ Each constraint entity $c_i$ is represented by constraint type and reference parameters indices which primitive(s) must adhere to it. 

\textbf{Engineering Sketch Definition.} In the field of parametric CAD, engineering sketches are fundamental, serving as detailed blueprints for designing a range of objects from small components to large structures. These sketches are essential for converting conceptual ideas into precise, manufacturable designs. To ensure a standardized representation, sketches of varying dimensions, spanning from millimeters to meters, are uniformly positioned within a bounding box of 1-meter width at the origin. Each sketch consists of two key sequences: a sequence of primitives, $\mathcal{S}$, and a sequence of constraints, $\mathcal{C}$. 
%\\red{Please refer to Fig. 1 here and in the next paragraph.}

%We apply 6-bit uniform quantization to continuous primitive parameters, converting them into discrete variables.
We adopt the normalization and quantization methods for primitive parameters as outlined by~\cite{seff2021vitruvion}. A sketch primitive is expressed as $\mathcal{S} = (e_1, e_2, ..., e_m),$ where $m$ represents the number of entities in the sketch. Each entity $e_i$ is characterized by positional parameters $(p_1,..., p_k)$, where $p$ represents the normalized coordinates of points that constitute the entity. Sketches typically include three types of entities—lines, arcs, and circles. %, represented with two, three, and four points respectively. 
As illustrated in Figure~\ref{fig:intro}, all sketches are centrally positioned and normalized within a range of [1,64]. Lines, shown in blue, are depicted using two points: start and end point coordinates. Curves, shown in green, are characterized by three points: the start, end, and a mid-point on the curve. Circles, illustrated in red, are portrayed with four uniformly distributed points on the circle's circumference. This format allows for the interpretation of each sketch as a sequence of tokens. Constraints are similarly represented as primitives in $\mathcal{C} = (c_1, ..., c_n),$ with each constraint entity $c$ being defined by its type and the reference indices of parameters to which the primitives must conform.

\textbf{CAD AutoCompletion Task.} In addressing the existing CAD AutoCompletion task, which aims to automate routine CAD design procedures, we propose a new autoregressive generative model. This task involves completing a partially given sketch to form a fully-realized design. The mathematical formulation of the task is:
\begin{equation}
\setlength{\abovedisplayskip}{2pt}
\setlength{\belowdisplayskip}{2pt}
    \mathcal{L}(\Theta) = - \log p_{\Theta}(\mathcal{S}| \mathcal{S}_p) = - \sum_{i=j}^{m} \log p_\Theta(e_{i:m}| e_{1:i})
    \label{autocompletion}
\end{equation}
Here, $m$ is the total number of entities in the complete sketch $\mathcal{S}$, and $\mathcal{S}_{p}=(e_1, ..., e_i)$ is a partial sequence containing 20\% to 80\% of the primitive entities from $\mathcal{S}$. Our model's goal is to optimize the log-likelihood of completing the sketch $\mathcal{S}$ based on these partial sequences.

We employ open-source natural language pre-trained Transformer models for our generative model, with a particular emphasis on T5 models~\cite{raffel2020exploring}. Additionally, we explore finetuning with GPT-3.5~\cite{brown2020language}. Our results indicate significant cross-domain knowledge transfer capabilities in these pre-trained models, showcasing their effectiveness in the context of CAD design.

\textbf{CAD Autoconstrain Task.}
The CAD autoconstrain task aims to autoregressively generate a set of constraints based on given geometry primitives. We model the constraint model as 
\begin{equation}
\setlength{\abovedisplayskip}{2pt}
\setlength{\belowdisplayskip}{2pt}
    \mathcal{L}(\phi) = - \log p_\Phi(\mathcal{C}| \mathcal{S}) = - \sum_{i=1}^{n} \log  p_\Phi(C_{j:n}| C_{1:j},S)
    \label{autoconstraint}
\end{equation}
where $n$ is the number of constraints, and each $\mathcal{C}_i$ is represented by a tuple of tokens indicating its constraint type and corresponding primitive entity parameters. Like autocompletion task, the autoconstrain model is trained to maximize the log-likelihood of generated tokens with respect to the ground truth. 

% \begin{equation}
%      \mathcal{L}(\phi) = - \log p(\mathcal{S}| \mathcal{S}_p; \Theta)
% \end{equation}
%\Amir{we can use this if we decide to write the total loss}

Aligned with \cite{seff2021vitruvion}, we focus on 13 constraint types, which are coincident, parallel, and so on. Further details about these constraints are provided in the Supplementary.
%\red{(maybe we should list all 13 constraints. Also, it is not clear what is a constraint. It should be illustrated in Fig. 1, and refer to the figure.)}. 


\textbf{Evaluation Metrics.} To quantitatively assess CAD generation models, we introduce three CAD-specific metrics: \textit{Sketch Accuracy}, \textit{Entity Accuracy}, and \textit{CAD F1}. 

\textit{Sketch Accuracy} measures the probability of correctly generating the entire remaining sketch ($N_s$), with $N$ being the total number of sketches in the test set. \textit{Entity Accuracy} evaluates the likelihood of correctly generating at least one entity in the ground truth ($N_e$). They are calculated as:
% $$ \small \text{Sketch Accuracy} = \frac{N_s}{N}, \quad \text{Entity Accuracy} = \frac{N_e}{N}$$
{\small
\[
\textit{Sketch Accuracy} = \frac{N_s}{N}, \quad \textit{Entity Accuracy} = \frac{N_e}{N}
\]
}
\textit{CAD F1} is a harmonic mean of precision and recall for each sketch, averaged over the dataset:

{\small
\[
\textit{CAD F1} = \frac{1}{N} \sum^{N}_{i=1} \frac{2 \times \text{sketch precision} \times \text{sketch recall}}{(\text{sketch precision} + \text{sketch recall})}
\]
}
% {\footnotesize
% \[
% \text{sketch precision} = \frac{n_c}{n_p}, \quad \text{sketch recall} = \frac{n_c}{m},
% \]
% }
where $\textit{sketch precision} = \frac{n_c}{n_p}$, $\textit{sketch recall} = \frac{n_c}{m}$, $n_c$ is the count of correct entities in the completed sketch, $n_p$ is the total number of entities predicted, and $m$ is the number of entities in the original sketch (ground truth).



==> sections/conclusion.tex <==
\section{Conclusion}
In this study, we introduce CadVLM, an innovative end-to-end vision-language model tailored for modeling parametric CAD sketches, which are pivotal in modern mechanical design. CadVLM harnesses the commonsense knowledge and reasoning abilities inherent in large language models, enabling it to adeptly handle the complex geometric reasoning required for CAD sketches. Our experimental results demonstrate that CadVLM outperforms existing state-of-the-art models in both autocompletion and autoconstraint tasks, highlighting the potent enhancement that pre-trained models bring to CAD construction.
% We are currently compiling a comprehensive, high-quality CAD sketch dataset, which we anticipate will serve as a superior benchmark for all models in this domain.
%Additionally, we observed limited performance from decoder-only models in our framework. Moving forward, we plan to incorporate open-source decoder-only models, such as LlaMa2~\cite{touvron2023llama}, for a more rigorous comparison and to further validate the efficacy of our approach.

==> sections/experiments.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{cccc}
\toprule
\multicolumn{1}{c|}{Model} & \multicolumn{1}{c}{Ske-Acc} & \multicolumn{1}{c}{Ent-Acc} & CAD-F1 \\ \hline
\multicolumn{1}{c|}{Vitruvion}          & 3.0\%  & 40.7\% & 11.3\% \\ \hline
\multicolumn{1}{c|}{ChatGPT-15\%}       & 6.8\%  & 41.3\% & 21.2\% \\
\multicolumn{1}{c|}{ChatGPT-7\%}        & 7.6\%  & 43.8\% & 22.2\% \\ 
\multicolumn{1}{c|}{ChatGPT-1\%}        & 6.5\%  & 43.7\% & 22.5\% \\ \hline
\multicolumn{1}{c|}{CadVLM-Text}        & 21.2\%  & 66.7\% & 42.8\% \\ 
\multicolumn{1}{c|}{CadVLM-w/o-IDL}     & 22.6\% & 68.4\% & 44.2\%\\ 
\multicolumn{1}{c|}{CadVLM-w/o-ITC}     & 22.8\% & 67.6\% & 43.9\% \\ 
\multicolumn{1}{c|}{CadVLM-w/o-IDL\&ITC} & 23.0\% & 67.7\% & 44.1\% \\ \hline
\multicolumn{1}{c|}{\textbf{CadVLM}}    & \textbf{23.8\%} & \textbf{68.3\%} & \textbf{45.2\%} \\ \hline
\end{tabular}
\caption{Quantitative sketch generative model comparison results for CAD autocompletion task. Ske-Acc means the probability of generating the correct full remaining sketch and Ent-Acc means the probability of generating at least one entity of the ground truth. \textbf{Bold} shows the best results of each metric. For all metrics the higher the better.}
\label{tab:autocompletion}
\end{table}
\begin{table}[h]
\small
\centering
\begin{tabular}{cccc}
\toprule
\multicolumn{1}{c|}{Model} & \multicolumn{1}{c}{Ske-Acc} & \multicolumn{1}{c}{Ent-Acc} & CAD-F1 \\ \hline
%\multicolumn{1}{c|}{}      & \multicolumn{3}{c}{CAD Autoconstraint} \\ \hline
\multicolumn{1}{c|}{SketchGraphs}       & 0.48\% & 93.0\% & 42.0\% \\ \hline
\multicolumn{1}{c|}{Vitruvion}          & 10.7\% & 94.6\% & 71.6\% \\ \hline
\multicolumn{1}{c|}{CadVLM-Text}        & 11.5\% & 95.0\% & 72.6\% \\ 
\multicolumn{1}{c|}{CadVLM-w/o-IDL}     & 11.3\% & 94.9\% & 73.8\% \\ 
\multicolumn{1}{c|}{CadVLM-w/o-IDL\&ITC} & \textbf{12.1\%} & \textbf{95.4\%} & \textbf{74.5\%} \\ \hline
\multicolumn{1}{c|}{\textbf{CadVLM}}    & 11.3\% & 94.9\% & 73.8\% \\ 
\toprule
\end{tabular}
\caption{Quantitative sketch generative model comparison results for CAD autoconstraint task. For all metrics higher is better.}
\label{tab:autoconstraint}
\vspace{-4mm}
\end{table}

\begin{figure*}[ht]
    \centering
    \includegraphics[scale=0.5]{cvpr2023-author_kit-v1_1-1/latex/sections/samples_results.pdf}
    \caption{Comparative Analysis of Autocompletion in CAD Design. Top row: Random samples from the SketchGraphs dataset. Second row: Initial input entities serving as the primer for the autocompletion task. Third and fourth row: Autocompletion results produced by Vitruvion and CadVLM.} %\red{(We should use 1st row, 2nd row, etc. You have 4 rows.)}} %The arrow indicates sketch precision of each CadVLM output sample, decreasing from 100\%(exactly matched) to 0\%(totally unmatched).}
    \label{fig:samples}
    \vspace{-5mm}
\end{figure*}

\section{Experiments}
We conduct extensive experiments and ablation studies on CadVLM for the CAD autocompletion and autoconstraint tasks. Quantitative assessment is conducted by measuring Entity Accuracy, Sketch Accuracy, and CAD F1. 
%\red{You mean CAD Precision, CAD Recall, and CAD F1?}. 
%We also evaluate the CadVLM's performance for image-conditioned Primitive generation tasks.

\subsection{Experimental settings}

\textbf{Dataset} We use the SketchGraphs~\cite{seff2020sketchgraphs} dataset for all our experiments, consisting of 15 million CAD sketches collected from Onshape\footnote{https://www.onshape.com}. Referring to~\cite{seff2021vitruvion}, we use the filtered version and further deduplicate the dataset. After deduplication, the training, validation, and test set have 626,236, 22,031, 21,979 unique sketches correspondingly. The filtered sketches are restricted to sketches comprised of arcs, circles, and lines.
%See the Supplementary for more details about the dataset. 
To ensure a fair comparison, we normalize each sketch as in ~\cite{seff2021vitruvion}; specifically the quantized range of numerical tokens in the primitive sequence is $[1,64]$.

% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{c|c|cc}
% \toprule
% Model                      & Conditioned Image      & Ent-Acc         & CAD-F1          \\ 
% \hline
% \multirow{3}{*}{Vitruvion} & precise                  & 83.8\%                    & 35.8\%          \\ 
%                            & hand-drawn          & \textbf{84.2\%}            & \textbf{38.4\%} \\ 
%                            & noisy hand-drawn           & 83.2\%                   & 36.9\%          \\
%                            \hline
% \multirow{3}{*}{CadVLM}   & precise             & 98.0\%             & \textbf{62.7\%} \\ 
%                            & hand-drawn               & \textbf{99.4\%}                     & 60.1\% \\ 
%                            & noisy hand-drawn          & 94.4\%                      & 56.5\%         \\
% \toprule
% \end{tabular}
% \caption{Quantative results for image conditioned primitive generation. \textbf{Bold} represents the best results of all metrics.}
% \label{tab:image_cond}
% \end{table}

\begin{table}[t]
\centering
\begin{tabular}{c|c|c|c}
\toprule
Condioned Image                  & Model     & Ent-Acc         & CAD-F1          \\ \hline
\multirow{2}{*}{Precise}          & Vitruvion & 83.8\%          & 35.8\%          \\ \cline{2-4} 
                                  & CadVLM    & \textbf{98.0\%} & \textbf{62.7\%} \\ \hline
\multirow{2}{*}{Hand-drawn}       & Vitruvion & 84.2\%          & 38.4\%          \\ \cline{2-4} 
                                  & CadVLM    & \textbf{99.4\%} & \textbf{60.1\%} \\ \hline
\multirow{2}{*}{Noisy hand-drawn} & Vitruvion & 83.2\%          & 35.8\%          \\ \cline{2-4} 
                                  & CadVLM    & \textbf{94.4\%} & \textbf{56.5\%} \\ \toprule
\end{tabular}
\caption{Quantitative results for image conditioned primitive generation. \textbf{Bold} represents the best results of all metrics.}
\label{tab:image_cond}
\vspace{-3mm}
\end{table}

%\subsection{Baselines}
\textbf{Baselines} We evaluate several ablation and conditional variants of CadVLM as well as two SOTA CAD generative model baselines: \textbf{Vitruvion}~\cite{seff2021vitruvion} and \textbf{SketchGraphs}~\cite{seff2020sketchgraphs}.
% For CAD autocompletion task, we compare CadVLM with Vitruvion~\cite{seff2021vitruvion}, which is the SOTA CAD generative model.
% For CAD autoconstraint task, we compare CadVLM
Since SketchGraphs does not incorporate continuous primitive parameters such as coordinate value, we only compare with the CAD autoconstraint task.

%Limited by the high cost of ChatGPT finetuning, we only finetuned a small portion of the data (1\%, 7\% and 15\%). And we found that performance didn't change dramatically with the increase of data or training epochs. We assume the reason is that GPT3.5 is being finetuned using PEFT (e.g. LORA)~\cite{hu2021lora} methods.


%\subsection{Experimental settings}
\textbf{Settings} For the image encoder and decoder, we choose the encoder and decoder of state-of-the-art pre-trained ViT-MAE-base from~\cite{he2022masked}. Following~\cite{he2022masked} we set the patch size and stride both as 32. We render all sketch images with size of $224\times224\times3$.
For the text encoder and text decoder, we use the encoder and decoder of pre-trained CodeT5+~\cite{wang2023codet5+} correspondingly, which is an instruction-tuned code LLM with 770M parameters trained on various code datasets.
We train the autocompletion model and autoconstraint model both for 30 epochs, using the Adam optimizer with decoupled weight decay regularization~\cite{loshchilov2017decoupled}, with the learning rate set according to the  CosineAnnealingLR~\cite{loshchilov2016sgdr} scheduler. The initial learning rate is set to $3e-4$, with batch size 32. All our experiments are run using 8 NVIDIA A100 GPUs, and our models take between 30-40 hours to train.
% Remarkable performance on all three metrics is achieved with training for only 20 epochs. These results demonstrate that foundational pre-trained models can indeed aid in CAD representation and generation tasks.
In the CAD Autocompletion experiments, we randomly sample 20\%-80\% of sketch entities as input and aim to predict the remaining entities from the ground truth sketch.


\subsection{Quantitative comparison with baseline sketch generative models}
%\red{(We need to be careful to call some models as SOTA. Maybe just call them baselines. In the main content, you can say it is SOTA according to your knowledge.)}}
Table~\ref{tab:autocompletion} reports results on the \textbf{CAD Autocompletion} task. We find that Vitruvion achieves 3\% on Sketch Accuracy and 40.7\% on Entity Accuracy, meaning it can accurately predict 3\% of sketches and correctly identifies at least one entity in 40.7\% of sketches. Our CadVLM outperforms Virtruvion on Sketch Accuracy, Entity Accuracy, and CAD-F1 by 20.8\%, 28.3\%, and 39.9\% respectively. These results demonstrate the effectiveness of pre-trained foundational models and image modality. A closer examination of the qualitative results in Figure~\ref{fig:samples} reveals that Vitruvion produces many invalid results missing symmetric curves or lines. Sketches from CadVLM are better in terms of quality with more complex shapes and stronger symmetry. 

%the commonsense knowledge in pre-trained large language models can impressively improve geometry reasoning ability.
%For enhanced visualization of our results, Figure~\ref{fig:samples} presents randomly selected examples. These examples illustrate that CadVLM's outputs closely resemble the original sketches and Vitruvion hardly predicts sketches exactly correctly, which is consistent with the quantitative data in Table~\ref{tab:autoconstraint}. Notably, even in cases of imperfect outputs (e.g., the first and second examples on the left), CadVLM generates outputs that are meaningful and potentially valuable in practical CAD engineering applications.

\textbf{ChatGPT Series Model Finetune} To evaluate the ability of a general LLM on the CAD autocompletion task, we fine-tuned ChatGPT on three subsets of 15\%, 7\%, and 1\% of the SketchGraphs dataset. The results indicate that the ChatGPT-series outperforms Vitruvion on all three metrics, especially on Sketch Accuracy and CAD-F1. However, there was no significant performance improvements when finetuning on larger portions of the training dataset. One possible reason is we only finetune ChatGPT for less than 5 epochs due to training costs, making it hard for ChatGPT to adapt to CAD data.

\textbf{CadVLM variants} To better understand the source of performance gains, we conducted a comparative analysis of different variants of our proposed CadVLM: CadVLM-text, CadVLM-w/o-IDL, CadVLM-w/o-ITC, CadVLM-w/o-IDL\&ITC. CadVLM-text relies solely on the sketch primitive sequence text as its input, optimizing for language modeling loss. In contrast, CadVLM-w/o-IDL utilizes ITC and LM loss for its training objectives, CadVLM-w/o-ITC focuses on IDL and LM, and CadVLM-w/o-IDL\&ITC prioritizes only the LM objective. The findings reveal that CadVLM-Text underperforms compared to all other CadVLM variants across all three metrics, which underlines the value of the sketch image modality in providing diverse geometric information alongside sequence text.

Interestingly, CadVLM-w/o-IDL emerges as the superior performer among the CadVLM variants, highlighting the significance of aligning image and text embeddings in multimodal modeling. Incorporating Image Decoding Loss (IDL) further enhances the alignment between image and text embeddings, leading CadVLM to show a notable improvement in all three metrics.


For the \textbf{CAD Autoconstraint} task, as shown in Table~\ref{tab:autoconstraint}, SketchGraphs struggles to predict the whole sketch correctly, with only 0.48\% Sketch Accuracy. This suggests that relying solely on graph structures of sketches is insufficient for handling long sequences of sketch primitives. In contrast, Vitruvion achieves 10.7\% on Sketch Accuracy, showing the necessity to model primitives.
For the CAD Autoconstraint task it is less challenging to predict at least one constraint correctly but more challenging to accurately predicting all constraints, easily caused by potential data labelling inconsistencies. As is well-known, minor discrepancies in primitive values can drastically alter constraints, such as changing them from parallel to coincident.

The CadVLM series model exceeds the performance of both SketchGraphs and Vitruvion across all metrics. Notably, CadVLM-w/o-IDL\&ITC emerges as the top performer within the CadVLM series. This may be attributed to its more substantial text decoder, which enables the model to more effectively integrate knowledge from both primitives and images to inform geometric information.


\begin{figure*}[ht]
	\begin{minipage}{0.31\linewidth}
		% \vspace{3pt}
		\centerline{\includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/sections/ratio_ent_acc.pdf}}
		\centerline{(a)}
	\end{minipage}
	\begin{minipage}{0.31\linewidth}
		% \vspace{3pt}
		\centerline{\includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/sections/ratio_ske_acc.pdf}}
		\centerline{(b)}
	\end{minipage}
	\begin{minipage}{0.31\linewidth}
		% \vspace{3pt}
		\centerline{\includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/sections/ratio_f1_acc.pdf}}
		\centerline{(c)}
	\end{minipage}
	\caption{Effect of input entity ratio to (a) Entity Accuracy, (b) Sketch Accuracy, and (c) CAD F1.}
 %\red{(Enlarge the x y axis font size, reduce the width of this figure to save space.)}}
	\label{fig:ratiovsacc}
\vspace{-3mm}
\end{figure*}


\subsection{Ablation Study}
We conducted several ablation studies to assess the performance of CadVLM on image-conditioned primitive generation tasks and investigate the effectiveness of each component within CadVLM.

\textbf{Image Conditional Generation.} 
Following~\cite{seff2021vitruvion}, we conduct a series of experiments to evaluate the effectiveness of CadVLM modeling primitive sequences conditioned on the images of sketches. As designers may begin their designs with hand-drawn sketches before transitioning to CAD programs, accurately inferring parametric CAD from images or scans can dramatically reduce the effort of translating from rough paper sketches to the CAD model.

When conditioning only on sketch images, the text encoder of CadVLM is ignored. We only use the image encoder, image decoder, and text decoder. The overall model is trained to maximize the probability of the ground truth primitives portrayed in the image, conditioned on a sequence of patch embeddings.

The results of Table~\ref{tab:image_cond} show three kinds of sketch image rendering input to imitate different settings in the real world: precise renderings, rendering from the hand-drawn simulator of~\cite{seff2021vitruvion}, and renderings with random affine augmentations of the hand-drawn simulator. As both Vitruvion and CadVLM can seldom predict the sketch exactly correctly, we ignore Sketch Accuracy in our image conditional generation experiments. The results show that CadVLM outperforms Vitruvion on both Entity Accuracy and CAD F1. Vitruvion performs best on hand-drawn images with 83.8\% Entity Accuracy and 38.4\% CAD F1. While CadVLM achieves almost 99.4\% Entity Accuracy and 62.7\% CAD F1.
Conditioning on precise rendered images acheives the best performance.
% which is alignment with the human engineer. 
%We also draw some examples of different rendering methods.

\begin{table}[t]
\centering
\small
% \begin{tabularx}{\columnwidth}{@{}c|ccc@{}}
\begin{tabular}{c|ccc}
\toprule
Model            & Ent-Acc     & Ske-Acc        & CAD-F1 \\ 
\midrule
CadVLM-Text                 & 66.7\%      & 21.2\%         & 42.8\% \\
w/-Inductive Bias       & 67.5\%      & 22.2\%         & 43.7\% \\ 
\bottomrule
\end{tabular}
\caption{Effect of adding the inductive bias of entity-level embeddings to the sketch sequence.}
\vspace{-5mm}
\label{tab:inductive_bias}
\end{table}

\textbf{Entity Level Modelling.}
As described earlier, each CAD sketch is comprised of multiple entities. We considered adding this inductive bias to the model by processing each entity separately and then combining their embeddings with the initial sequence of all sketch tokens. For this purpose, we first prepend a special token \textlangle ENTITY\textrangle~to each of the entity input sequences. Subsequently, the entities from all the sketches in the batch are fed into the model's encoder in parallel.
% Since the length of each tokenized entity is small, with a maximum of nearly 20 for a circle depending on the tokenizer, the batch size can be larger than . 
Next, the embeddings of each entity are gathered for each sketch. For each sketch, we concatenate these embeddings with the original sequence tokens using another special token \textlangle TOKEN\textrangle~as a delimiter for the second part of the sequence. The decoder remains unchanged. As shown in Table \ref{tab:inductive_bias}, incorporating this inductive bias increases computation and memory demands while only marginally enhancing the performance.

% Next we prepend another special token  to these sequence of embeddings so the model understands that sketch is the input (i.e. next level of hierarchy). The decoder is unchanged. This approach hugely reduces input token length to the number of entities instead of number of all the tokens in the sketch. One of the recent articles that studies similar approaches for efficiency is ~\cite{yu2023megabyte}. 
% You can find the results in Table~\ref{tab: different language models}. As you can see increasing the efficiency comes at a small cost of slightly worse performance. However, our group is moving towards complicated manufacturing sketches and this proposed method can be very helpful in training models tailored for complex sketches. 

% Since CAD-autocomplete is relatively a novel task, the current public datasets are relatively simple. However, in many applications including manufacturing industries, CAD drawings are complex so the number of input tokens can become complete. In this section, we briefly discuss our efforts to tackle this issue. As discussed, each sketch consists of multiple entities. Each entity solely has a representation that can be processed separately. So, one way to process the whole sketch is to pass all the entities to the model encoder in parallel and then feed the sequence of their corresponding representations to an encoder-decoder model. 


% One of the recent articles that studied input patching for the sake of efficiency is ~\cite{yu2023megabyte}.

\textbf{Impact of different input entity ratios for CAD autocompletion.} To explore the impact of different input entity ratios for CAD autocompletion, we further test CAD autocompletion results with different input entity ratios: 20\%, 40\%, 60\%, and 80\%. Compared with the experiments in Sec 5.4, we specify the sampled ratio of input entities. As shown in Figure~\ref{fig:ratiovsacc}, CadVLM outperforms Vitruvion on all input entity ratios. In particular, CadVLM achieves 73.8\% Entity Accuracy, 49.5\% Sketch Accuracy, and 62.7\% CAD F1 when given 80\% of entities as input. For the hardest setting when given only 20\% of entities as input, CadVLM can still achieve 43.9\% Entity Accuracy and 16.9\% CAD-F1, which proves that CadVLM has great potential to be used in real world settings.

\begin{table}[t]
\centering
\small
\begin{tabular}{c|cccc}
\toprule
Model   & \#Parameter                  & Ent-Acc     & Ske-Acc        & CAD-F1          \\ 
\hline

CodeT5+   & 220M &  66.5\%            & 21.5\%               &   42.9\% \\
$\text{CodeT5+}^*$ & 220M & 65.0\%             & 18.9\%             & 40.3\% \\ 

CodeT5+   & 770M &  66.7\%            & 21.2\%              &   42.8\% \\
ByT5-base & 580M & 66.9\%                  & 22.0\%                    & 43.1\%          \\ 

ByT5-large & 1.2B & 66.8\%                  & 20.6\%                    & 41.9\%          \\ 

                            
T5-base   & 223M & 66.2\%             & 20.2\%             & 41.7\% \\ 

T5-large   & 783M & 66.8\%             & 21.2\%             & 42.6\% \\ 

\toprule
\end{tabular}
\caption{Effect of using different architectures for CadVLM-Text. CodeT5+ 770M is the encoder-decoder for text we use in our main experiments. CodeT5+* is the result of training from scratch rather than pre-trained. }
\label{tab: different language models}
\vspace{-5mm}
\end{table}
\textbf{Effect of using different language models for text encoder and decoder.} To better compare the performance of different text encoder-decoder, we experiment using different pre-trained foundation models as text encoder and decoder. To eliminate the influence of the image encoder and decoder, we only consider the CadVLM-Text variant. For the choice of text encoder and decoder, we also compare the performance of different Encoder-Decoder pre-trained language models on CAD autocompletion. The T5 family of models are among the most recognized and widely used encoder-decoder models in the open-source community. Therefore, we experimented with T5 ~\cite{raffel2020exploring}, ByT5 ~\cite{xue2022byt5} and CodeT5+ ~\cite{wang2023codet5+}. The results are shown in Table \ref{tab: different language models}. The effect of model size is clear for T5 and CodeT5+ but not ByT5. Also, The cost-benefit of solely making the model bigger becomes less favorable over time as the improvements in performance start to plateau. Another observation is that, because of the nature of the data which is closer to a code sequence than natural language, CodeT5+, which is fine-tuned on code, exhibits better performance. 

We also trained CodeT5+ from scratch to examine the impact of pre-training on natural language and code. As evidenced in Table~\ref{tab: different language models}, training from scratch falls short in all three metrics. Additionally, training from scratch converged much slower than finetuning. Despite the fact that our representation of sketches as code is relatively unique and not found in natural language, the rules and token embeddings learned from text are very helpful for domain adaptation. 

==> sections/introduction.tex <==
%%%%%%%%% BODY TEXT
% \begin{figure*}[!h]
%     \centering
%     \includegraphics[width=0.99\textwidth]{cvpr2023-author_kit-v1_1-1/latex/sections/Intro-v2.pdf}
%     \caption{For the CAD autocompletion task, our multi-modal \textbf{CadVLM} model (b) receives partial CAD entities as both image and text input (a) and generates the remaining sketch entities as output (c). The complete sketch, with optional predicted constraints, can then be used in CAD software (d) to form 3D shapes (e).   }
%     % The output images here are rendered by output text, which aligns with inference. During training, the output images are generated by image decoder.
%     %A key distinction from image inpainting is that the output for CAD autocompletion is sketch primitive incorporating parameterized entity position.}
%     \label{fig:intro}
% \end{figure*}

\section{Introduction}
\label{sec:intro}
% Parametric Computer-Aided Design (CAD) stands as the prevailing paradigm in the field of mechanical engineering for crafting modern physical objects. The creation of engineering sketches necessitates a profound understanding of geometry and often relies heavily on a substantial repository of reference CAD designs.

Parametric Computer-Aided Design (CAD) is a cornerstone in mechanical engineering, playing a pivotal role in the development of modern physical objects. This method relies on precise geometric parameters to shape and manipulate 3D models, making it indispensable in industrial design. The significance of parametric CAD lies in its ability to accurately represent complex designs,  crucial to the integrity and functionality of engineered products. Recognizing the importance of CAD in industrial design, there is a strong motivation to advance CAD generation. Enhancing CAD processes with automated tools not only promises to streamline design workflows but also to foster innovation by enabling more complex and precise designs.

% In the CAD community, `engineering sketches' are used to form the 2D basis of parametric CAD, by which 3D shapes are lifed into 3D using modeling operations such as \textit{extrude} and \textit{revolve}. These sketches consist of geometric primitives (lines, arcs, circles etc.), their associated parameters (coordinates, radius, etc.), along with a set of constraints which govern the relations between these primitive such as coincidence, parallelism, and symmetry. Design using CAD tools can be challenging and tedious for engineers. Although general motifs may be repeated across related parts in a design, the CAD tools of today are largely unaware of repeat design patterns, resulting in repetitive work for engineers. With the help of deep learning, capturing patterns in CAD sketches has the potential to speed up manual design by automatically completing both the geometry and constrains found in engineering sketches.
%In addition, engineers often meet the situation when given part of the sketch to finish it. Automatically autocomplete the sketch can hugely enhance the efficiency of CAD designing.

The integration of deep learning into CAD presents an exciting opportunity to revolutionize this field. Engineering sketches,  which are foundational 2D blueprints in parametric CAD, are ripe for innovation through machine learning techniques. By applying deep learning, particularly multimodal approaches, we can capture and replicate the intricate patterns and geometric relationships inherent in these sketches. Our work introduces a significant advancement in CAD design: a novel Multimodal Transformer-based Generative model, meticulously crafted for CAD generation. This model uniquely incorporates both visual and textual data, utilizing the strengths of deep learning to better understand and create intricate CAD designs. By integrating these modalities, we aim to enhance the precision and efficiency of CAD generation, marking a notable step forward in the application of AI in industrial design.

Recent research has focused on generative modeling of engineering sketches, with an emphasis on Transformer-based architectures ~\cite{vaswani2017attention}, as seen in ~\cite{seff2020sketchgraphs,seff2021vitruvion, willis2021engineering}. These methods often employ graph structures or attention mechanisms to learn from sketch information. However, restricted data availability and limited commonsense understanding hinder their ability to grasp complex geometric reasoning in engineering sketches.
% Such shortcomings pose significant challenges in the practical application of these models in engineering design.

Large Language Models (LLMs) have garnered recognition for their versatile application across diverse domains. They excel in commonsense reasoning and emergent problem-solving across various fields, including natural language processing, mathematics, and medical sciences~\cite{singhal2022large,azerbayev2023llemma, luo2023wizardmath, singhal2023towards,floridi2020gpt, chen2022pali,zha2023tablegpt}.
 % and their adeptness in processing a range of data types.
% Their potential in the realm of engineering sketch design is particularly intriguing.
Engineering sketches can be conceptualized as strings that depict points and connections, which align seamlessly with the proficiencies of LLMs. Moreover, aligning sketch images with textual descriptions can significantly enhance the performance of language models on specific domains~\cite{li2022blip}. 
In parametric CAD design, which demands a deep understanding of complex interactions and constraints, the strengths of LLMs are especially beneficial.

In this work, we leverage the capabilities of pre-trained LLMs to develop a generative model tailored for parametric CAD, addressing the limitations of the existing methods. We introduce \textbf{CadVLM}, a CAD Vision Language Model, featuring a multimodal asymmetric encoder-decoder framework. CadVLM stands out by processing engineering sketches both linguistically, through token sequences representing sketch geometry and constraints, and visually, via rendered sketch images. To the best of our knowledge, CadVLM is the first generative model to utilize pre-trained vision and language models for CAD sketches, which is capable of addressing different CAD representation learning tasks such as CAD autocompletion, CAD autoconstraint, and image conditional generation tasks.
Our contributions are threefold:
\begin{itemize}
\item We propose CadVLM, a novel CAD Vision-Language Model, for simultaneously modeling engineering sketches as both language and images. This model facilitates not only sketch autocompletion but also CAD autoconstraint, which are automatic geometry and constraint generation capabilities.
\item We introduce three evaluation metrics—Entity Accuracy, Sketch Accuracy, and CAD F1 score—to quantitatively assess the quality of generated CAD sketches.
\item Through extensive experiments on the SketchGraphs dataset~\cite{seff2020sketchgraphs}, CadVLM demonstrates superior performance over all baseline models in CAD autocompletion and autoconstraint tasks.
\end{itemize}

% Large language models (LLM), renowned for their versatile abilities in various domains and their capability to process a plethora of data forms, present a promising avenue. On one hand, given that engineering sketches can be converted into a string format representing points and their connectivity, we scrutinize the potential of these models in engineering sketch design. And paired sketch images can be aligned with text for better image-grounded language models. On the other hand, LLMs have demonstrated commonsense and emergent reasoning abilities in natural language processing, math, and medical domains~\cite{singhal2022large,azerbayev2023llemma, luo2023wizardmath, singhal2023towards,floridi2020gpt, chen2022pali,zha2023tablegpt}. Construction of parametric CAD, relies heavily on complex reasoning of parametric relationships and constraints, while also depending on geometric understanding. 

% In this work we address the shortcomings of existing techniques by leveraging the abilities of pre-trained LLMs to build a generative model for parametric CAD. Specifically, we build a vision-language model for modeling engineering sketches as both language (sequences of tokens representing sketch geometry and constraint entities) and vision (rendered images of sketches). Our model, \textbf{CadVLM}, standing for CAD Vision Language Model, uses a multi-modal asymmetric encoder-decoder architecture, with interactive text and image modules.
% To the best of our knowledge this is the first generative model to represent CAD sketches using pre-trained vision-language models. 

% Our contributions are as follows:
% \begin{itemize}
%     \item We propose a CAD Vision-Language Model(CadVLM) for modeling engineering sketches as both language and images at the same time, which can not only perform sketch autocompletion but also 
%     CAD autoconstraint.%ground image information during both encoding and generation.

%     \item We introduce three novel evaluation metrics for CAD generative models: Entity Accuracy, Sketch Accuracy, and CAD F1 score, which can quantitatively measure the quality of generated CAD sketches.
    
%     \item We perform extensive experiments on the SketchGraphs dataset~\cite{seff2020sketchgraphs} for the CAD autocompletion and CAD autoconstraint tasks.  CadVLM achieves state-of-the-art performance on all baselines.
% \end{itemize}

% \begin{enumerate}
% \item We propose a CAD Visual Language Model(CadVLM) for modeling CAD sketch parameters and images at the same time, which can not only perform sketch autocompletion but also ground image information during both encoding and generation.
%     \item We introduce three novel evaluation metrics for CAD generative models: Entity Accuracy, Sketch Accuracy, and CAD F1 score, which can quantitatively measure the quality of generated CAD sketches.
% \item We perform extensive experiments on SketchGraphs dataset for CAD autocompletion and CAD autoconstraint tasks,  CadVLM achieves state-of-the-art performance over all baselines.
% \end{enumerate}



==> sections/method.tex <==
\section{CadVLM: A Vision Language Model for CAD Generation}
\label{sec:method}
In this section, we delve into the specifics of our CAD Vision Language Model (CadVLM), employing the CAD autocompletion task as an illustrative example. In our approach, the sequence of sketch primitives $\mathcal{S}$ is interpreted akin to language text, while the corresponding visual representation of the sketch is treated as image $I$.

\subsection{Network Framework}

CadVLM is structured as an asymmetrical encoder-decoder architecture, featuring a two-stream encoder, a text decoder based on a language model, and a lightweight image decoder for constructing the autocompleted image. This design is depicted in Figure~\ref{fig:architecture}. The two-stream encoder is tailored to process dual-modal inputs: a vision sub-encoder for the sketch image $I$ and a text sub-encoder for the prefix sequence of sketch primitives $S_p$. For text decoding, we employ a causal language transformer model, which autoregressively generates the output, i.e., the autocompleted sketch. Finally, the image decoder utilizes the latent representation tokens to construct the visual representation of the autocompleted sketch.

\textbf{Vision Encoding Stream.}
To encode partial sketch images and harness the capabilities of an existing large vision autoencoder model, we employ a pre-trained vision transformer (ViT)\cite{he2022masked} for extracting vision features. To bridge the gap between CAD images and natural images typically processed by ViT, we fine-tune the model on the SketchGraphs dataset. This fine-tuning involves a one-epoch image reconstruction task, with a 75\% masking ratio, specifically tailored for CAD sketch data. Figure~\ref{fig:vitmae} illustrates the image reconstruction outcomes using both the original pre-trained ViT-MAE and the version fine-tuned on the SketchGraphs dataset. After finetuning, ViT-MAE shows enhanced representational performance for CAD sketches.

However, it's important to note that while some reconstructed sketches are notably accurate, they do not fully meet the requirements for parametric CAD engineering due to the vagueness and lack of parameterization in the entities. To bring image and text features to the same embedding space, we integrate a down-sampling layer and a lightweight projection module atop the vision encoder.

\textbf{Text Encoding Stream.} 
Treating the sketch primitive sequence as textual data, we first tokenize this sequence to derive a series of text tokens $T={t_1,t_2,...,t_l}$. These tokens are then processed using the encoder of a pre-trained language model, effectively encoding the sketch information in a textual format.

\begin{figure}
    \centering
    \includegraphics[scale=0.75]{cvpr2023-author_kit-v1_1-1/latex/sections/vitmae.pdf}
    \caption{CAD image reconstruction results by ViTMAE. (a) Input sketches, (b) masked sketches with the mask ratio of 75\%, reconstructed results using a (c) pre-trained and (d) further fine-tuned ViT-MAE.}
    %\red{(The title is confusing. What do you mean? Please revise it.)}}
    % CAD image reconstruction results of (c)pre-trained and (d)further fine-tuned ViT-MAE on Sketchgraphs dataset. (a) shows the original sketches and (b) are the masked sketches with the mask ratio 75\%.
    \label{fig:vitmae}
    \vspace{-4mm}
\end{figure}

\textbf{Text-grounded Vision Decoding Stream.} This stream is dedicated to constructing the autocompleted pixels, mapping the fused image and text representation to the pixel-level sketch image.  The input for the vision decoder comprises the fused image and text embeddings, augmented with adaptively masked token patches to keep the same patch size as input image. This construction process ensures that the vision embedding is grounded by textual information and also enhances the text representation.

\textbf{Image-grounded Text Decoding Stream.} In alignment with Equations~\ref{autocompletion} and \ref{autoconstraint}, we conceptualize autocompletion as a conditional text generation process. Within this framework, the combined image and text embeddings serve as inputs to the decoder of a language model. This decoder is capable of autoregressively generating the required output. Notably, the parameters of this language model are initialized from a pre-trained model, which itself has undergone extensive pre-training on vast datasets of code~\cite{wang2023codet5+}, enhancing its effectiveness in this context.

\subsection{Training Objectives}
As shown in Figure~\ref{fig:architecture},  we jointly optimize three distinct objectives during training: one focused on understanding and two on generation.

\textbf{Image-Text Contrastive Loss (ITC)} is employed to activate the unimodal encoders, following the approach in~\cite{li2022blip}. This loss function aligns the visual and textual feature spaces by ensuring that positive image-text pairs have similar representations, while contrasting with negative pairs. Such a contrastive approach has been instrumental in enhancing multimodal model training~\cite{radford2021learning, li2021align}, not only improving the alignment of visual and language features but also accelerating the convergence during training.
The image-text contrastive loss is defined as the cross-entropy between the similarity $p$ of image(I) text(T) embedding pairs and ground-truth one-hot similarity $y$ (array from [0,N], N is the number of samples), formulated as: 
\begin{equation}
    p = \frac{\text{exp}(s(I, T))}{\sum\limits_{i,j}^{N} \text{exp} (s(I_{i}, T_{j}))},  \mathcal{L}_{ITC} = \text{Cross-Entropy}(y,p).
\end{equation}


% \begin{equation}
%     \setlength{\belowdisplayskip}{52pt}
%     % \mathcal{L}_{ITC} = -\log \left( \frac{\exp(s(I, T))}{\sum_{T'} \exp(s(I, T'))} \right)
%     \mathcal{L}_{ITC} =  \left( \frac{\exp(s(I, T))}{\sum\limits_{T'} \exp(s(I, T'))} \right)
%     \vspace{1mm}
% \end{equation}
\textbf{Image Decoding Loss (IDL)} is responsible for constructing autocompletion sketch images. This process involves translating the fused visual and textual information into pixel values for each patch. IDL employs a mean squared error (MSE) loss, similarly to the approach in ViTMAE~\cite{he2022masked}, comparing the autocompleted sketch images with their ground-truth counterparts at the pixel level. The Image decoding loss can be formulated as:
\begin{equation}
    \mathcal{L}_{IDL} = \frac{1}{n} \sum_{i=1}^{n} (Y_i - \hat{Y}_i)^2,
\end{equation}
where $n$ is the number of total pixels, $Y_i$ is the ground-truth pixel value of $i$-th pixel, and $\hat{Y}_i$ is the output pixel value correspondingly.

\textbf{Language Modeling Loss (LM)} is designed to generate text-like autocompletion sketches, focusing on constraint sequences and utilizing the image-grounded text decoder. It optimizes a cross-entropy loss to maximize the likelihood described in Equation~\ref{autocompletion}. LM endows the model with the capability to transform fused multimodal information into coherent autocompletion sketch sequences. For the CAD autoconstraint task, we use Equation~\ref{autoconstraint} as the language modeling loss.

The full training objective of CadVLM is:
% \begin{equation}
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
%     \mathcal{L} = \mathcal{L}_{ITC} +\mathcal{L}_{LM} +\mathcal{L}_{IDL}     
% \end{equation}

\begin{equation}
\setlength{\abovedisplayskip}{2pt}
\setlength{\belowdisplayskip}{2pt}
    \mathcal{L} = \mathcal{L}_{ITC} +\mathcal{L}_{LM} +\mathcal{L}_{IDL}     
\end{equation}

% $$$$
%\red{(I think it is better to add some math formulas to represent the losses formally. Also, it is not clear how the 3 objectives are combined together. You need to add a formula to show the combination.)}

% \begin{table*}[h]
% \centering
% \begin{tabular}{cccccc}
% \toprule
% \multicolumn{1}{c|}{Model}              & \multicolumn{1}{c|}{Ske-Acc} & \multicolumn{1}{c|}{Ent-Acc} & \multicolumn{1}{c|}{CAD-Recall} & \multicolumn{1}{c|}{CAD-Precision} & CAD-F1 \\ \hline
% \multicolumn{1}{c|}{}                   & \multicolumn{5}{c}{CAD Autocompletion}                                                                                                      \\ \hline
% \multicolumn{1}{c|}{Vitruvion}          & \multicolumn{1}{c|}{3\%}     & \multicolumn{1}{c|}{40.7\%}  & \multicolumn{1}{c|}{52.1\%}           & \multicolumn{1}{c|}{49.6\%}              & 11.3\% \\ \hline
% \multicolumn{1}{c|}{ChatGPT-15\%}          & \multicolumn{1}{c|}{6.8\%}     & \multicolumn{1}{c|}{41.3\%}  & \multicolumn{1}{c|}{}           & \multicolumn{1}{c|}{}              & 21.2\% \\
% \multicolumn{1}{c|}{ChatGPT-7\%}          & \multicolumn{1}{c|}{7.6\%}     & \multicolumn{1}{c|}{43.8\%}  & \multicolumn{1}{c|}{}           & \multicolumn{1}{c|}{}              & 22.2\% \\ 
% \multicolumn{1}{c|}{ChatGPT-1\%}          & \multicolumn{1}{c|}{6.5\%}     & \multicolumn{1}{c|}{43.7\%}  & \multicolumn{1}{c|}{}           & \multicolumn{1}{c|}{}              & 22.5\% \\ \hline

% \multicolumn{1}{c|}{CadVLM-Text}   & \multicolumn{1}{c|}{22\%}    & \multicolumn{1}{c|}{67.3\%}  & \multicolumn{1}{c|}{}           & \multicolumn{1}{c|}{}              & 43.4\% \\ 
% %\multicolumn{1}{c|}{CadVLM-Image}   & \multicolumn{1}{c|}{ }    & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}           & \multicolumn{1}{c|}{} \\ \hline
% \multicolumn{1}{c|}{CadVLM-w/o-IDL}   & \multicolumn{1}{c|}{22.6\%}    & \multicolumn{1}{c|}{68.4\%}  & \multicolumn{1}{c|}{43.7\%}           & \multicolumn{1}{c|}{44.9\%} & 44.2\%\\ 
% \multicolumn{1}{c|}{CadVLM-w/o-ITC}   & \multicolumn{1}{c|}{22.8\%}    & \multicolumn{1}{c|}{67.6\%}  & \multicolumn{1}{c|}{}           & \multicolumn{1}{c|}{} & 43.9\% \\ 
% \multicolumn{1}{c|}{CadVLM-w/o-IDL\&ITC}   & \multicolumn{1}{c|}{23.0\%}    & \multicolumn{1}{c|}{67.7\%}  & \multicolumn{1}{c|}{47.7\%}           & \multicolumn{1}{c|}{46.7\%} & 44.1\% \\ \hline
% %\multicolumn{1}{c|}{CadVLM-frozen}   & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}           & \multicolumn{1}{c|}{} &  \\ \hline
% \multicolumn{1}{c|}{\textbf{CadVLM}} & \multicolumn{1}{c|}{23.8\%}  & \multicolumn{1}{c|}{68.3\%}  & \multicolumn{1}{c|}{48.1\%}           & \multicolumn{1}{c|}{46.1\%}             & 45.2\% \\ \hline
% \multicolumn{1}{l}{}                    & \multicolumn{5}{c}{CAD Autoconstraint}                                                                                                      \\ \hline
% \multicolumn{1}{c|}{SketchGraphs}       & \multicolumn{1}{c|}{0.48\%}  & \multicolumn{1}{c|}{93\%}    & \multicolumn{1}{c|}{41.9\%}     & \multicolumn{1}{c|}{42.1\%}        & 42.0\% \\ \hline
% \multicolumn{1}{c|}{Vitruvion}          & \multicolumn{1}{c|}{10.7\%}    & \multicolumn{1}{c|}{94.6\%}  & \multicolumn{1}{c|}{\textbf{78.6\%}}     & \multicolumn{1}{c|}{\textbf{76.8\%}}        & 71.6\% \\ \hline
% \multicolumn{1}{c|}{CadVLM-Text}   & \multicolumn{1}{c|}{11.5\%}    & \multicolumn{1}{c|}{\textbf{95.0\%}}  & \multicolumn{1}{c|}{74.9\%}           & \multicolumn{1}{c|}{73.4\%}     & 72.6\% \\ 
% \multicolumn{1}{c|}{CadVLM-w/o-IDL}   & \multicolumn{1}{c|}{11.3\%}        & \multicolumn{1}{c|}{94.9\%}        & \multicolumn{1}{c|}{75.6\%}         & \multicolumn{1}{c|}{76.1\%}      & 73.8\% \\ 
% % \multicolumn{1}{c|}{CadVLM-w/o-ITC}   & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}           & \multicolumn{1}{c|}{} &  \\ \hline
% \multicolumn{1}{c|}{CadVLM-w/o-IDL\&ITC}   & \multicolumn{1}{c|}{\textbf{12.1\%}}    & \multicolumn{1}{c|}{95.4\%}  & \multicolumn{1}{c|}{77.4\%}           & \multicolumn{1}{c|}{76.0\%} & \textbf{74.5\%} \\ \hline
% %\multicolumn{1}{c|}{CadVLM-frozen}   & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}           & \multicolumn{1}{c|}{} &  \\ \hline
% \multicolumn{1}{c|}{\textbf{CadVLM}} & \multicolumn{1}{c|}{11.3\%}        & \multicolumn{1}{c|}{94.9\%}        & \multicolumn{1}{c|}{75.6\%}         & \multicolumn{1}{c|}{76.1\%}      & 73.8\%    \\ 
% \toprule
% \end{tabular}
% \caption{Quantitative sketch generative model comparison results for CAD autocompletion task and CAD autoconstraint task. }
% \label{tab:comparison}
% \end{table*}



==> sections/related.tex <==
\section{Related Work}
\label{sec:relate_work}
% Engineering sketches are composed of geometric primitives (line segments, circles, etc.) with associated parameters (coordinates, radius, etc.) and constraints (symmetry, tangent, coincident etc.). These 2D sketches form the basis of 3D CAD and are lifted into 3D by modeling operations such as \textit{extrude} and \textit{revolve}.
\textbf{Vision Language Pre-Training.}
The great success of large language models (LLMs) such as BERT~\cite{kenton2019bert} and GPT~\cite{brown2020language} has drawn significant attention within the field of natural language processing and code generation domain. %ChatGPT, Codex, and GPT-4 from OpenAI have shown remarkable capabilities in various tasks, including text generation, question answering, code generation, and so on. However, specific details about their training and model weight parameters remain undisclosed. 
CodeT5+~\cite{wang2023codet5+} is a family of open-source encoder-decoder LLMs for code tasks, ranging from 220 million to 16 Billion parameters. 
Beyond single modality LLMs, multimodal foundation models have also exhibited enhanced performance in various vision-and-language tasks~\cite{radford2021learning, li2022blip}. Depending on downstream tasks, %different model architectures have been proposed, such as dual-encoder architecture~\cite{radford2021learning}, the fusion-encoder architecture~\cite{ebrahimi2023lanistr}, and the encoder-decoder architecture~\cite{yu2022coca, chen2022pali}. 
Various pre-training objectives have also been proposed like image-text contrastive learning~\cite{radford2021learning}, image-text matching~\cite{li2022blip}, and (masked) language modeling~\cite{li2022blip}.
For example, 
%CLIP~\cite{radford2021learning} directly aligns image representations with corresponding text representations using contrastive loss. Blip~\cite{li2022blip} pre-trains a multimodal mixture of encoder-decoder models on a dataset bootstrapped from large-scale noisy image-text pairs.
Flamingo~\cite{alayrac2022flamingo} integrates new cross-attention layers into the LLM to incorporate visual features, pre-training these layers on billions of image-text pairs.
Most recently,  developing domain-specific multimodality LLMs has gained momentum such as MedBLIP~\cite{chen2023medblip} and TableGPT~\cite{zha2023tablegpt}.

\paragraph{CAD Sketch Generation}
%2D engineering sketches are fundamental in CAD for designing and manufacturing mechanical parts. 
The recent availability of extensive engineering sketch datasets has facilitated the development of generative models that enhance traditional CAD workflows. The SketchGraphs~\cite{seff2020sketchgraphs} dataset, featuring 15 million parametric CAD sketches with detailed geometric constraint graphs, showcases primitive interrelations. The paper also introduces a baseline model using autoregressive message-passing networks for constraint graph generation, but it lacks primitive coordinate output, relying solely on constraint graphs and the Onshape solver for sketch configuration, thus limiting its utility in CAD autocompletion tasks.
%making it not a total match with the CAD autocomplete task. 
% due to the inherent limitations of message-passing networks,
 %Furthermore,  SketchGraphs can generate constraints for only one sketch at a time, hindering its application in handling large datasets typical in real-world engineering scenarios.
Ganin et al. \cite{ganin2021computeraided} proposed another large-scale CAD dataset containing over 4.7M parametric sketches from the Onshape public repository. However, limited by sketch format, this dataset has not been widely researched in the realm of CAD generative models.

Another line of work for generative modeling of CAD sketches is based on Transformer~\cite{willis2021engineering,wu2021deepcad, seff2021vitruvion, xu2023hierarchical}. Vitruvion~\cite{seff2021vitruvion} models both primitives and constraints, but its training on Transformer does not inherently include geometric knowledge. Furthermore, Vitruvion's major limitation lies in its lack of quantitative comparison in terms of CAD generation quality.
While CurveGen~\cite{willis2021engineering} tackles the problem of engineering sketch generation without considering sketch constraints like us, it struggles to generalize to few-shot samples. What's more, both Vitruvion and CurveGen face limitations in their model performance, making them challenging to deploy in practical CAD engineering applications. Recently, there has been some research about CAD construction sequences generation~\cite{xu2022skexgen,xu2023hierarchical}. However, these works cannot model sketch primitives to autocomplete parametric CAD sketches. As Vitruvion and SketchGraphs are current state-of-the-art models in CAD sketch representation learning, we compare CadVLM with the Vitruvion and SketchGraphs models on the CAD Autocompletion task and CAD Autoconstraint task quantitatively.
%\Amir{We are mentioning Curvegen but not reporting results}
%\hl{TODO: add a sentence about the baselines we chose and why}
%In this paper, we evaluate CadVLM on one of the largest publicly available constrained sketch datasets SketchGraphs~\cite{seff2020sketchgraphs}. 
Different from existing work, our method utilizes sketch image modality and commonsense knowledge in pre-trained foundation models, providing both sketch sequence textual and image information for sketch generation process.
% MedBLIP~\cite{chen2023medblip} pre-trains on electronic health records in the form of images and texts. TableGPT~\cite{zha2023tablegpt} aims to integrate tables, natural language, and commands within a singular LLM framework.

% To harness the potential of pre-trained foundational models in CAD generation, we propose an end-to-end vision-language model tailored for CAD sketch generation. This model benefits from the commonsense knowledge of pre-trained models and distinctively integrates CAD sketch image information with primitives. %can combine diverse knowledge beyond CAD training data(such as more general geometric information).
% To the best of our knowledge, CadVLM is the first to apply pre-trained vision language models for CAD generation, which  is capable of addressing different CAD representation learning tasks such as CAD autocompletion, CAD autoconstraint, and image conditional generation tasks.
